AutoAdapt: Automated Segmentation Network Search for Unsupervised Domain Adaptation

Neural network-based semantic segmentation has achieved remarkable results when large amounts of annotated data are available, that is, in the supervised case. However, such data is expensive to collect and so methods have been developed to adapt models trained on related, often synthetic data for which labels are readily available. Current adaptation approaches do not consider the dependence of the generalization/transferability of these models on network architecture. In this paper, we perform neural architecture search (NAS) to provide architecture-level perspective and analysis for domain adaptation. We identify the optimization gap that exists when searching architectures for unsupervised domain adaptation which makes this NAS problem uniquely difficult. We propose bridging this gap by using maximum mean discrepancy and regional weighted entropy to estimate the accuracy metric. Experimental results on several widely adopted benchmarks show that our proposed AutoAdapt framework indeed discovers architectures that improve the performance of a number of existing adaptation techniques.

==> tables/overview_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet15'
\begin{table}[t!]
%   \centering
  \resizebox{1.0\linewidth}{!}{%

    \begin{tabular}{l|cc|cc}
    \toprule
    Methods & Arch. Design & Adap. Apprc. & GTA5 & SYNTHIA\\
    \hline
    AdvEnt \cite{vu2019advent} & Manual & AT    & 43.8 & 48.0\\
    Auto-AdvEnt (Ours) & Search & AT    & \textbf{45.3} & \textbf{49.2}\\
    \hline
    IntraDA \cite{pan2020intrada} & Manual & SL    & 45.9 & 48.9\\
    Auto-IntraDA (Ours) & Search & SL    & \textbf{47.2} & \textbf{50.4}\\
    \hline
    CCM \cite{li2020ccm}& Manual & ST    & 49.9 & 52.9 \\
    Auto-CCM (Ours) & Search & ST    & \textbf{50.2} & \textbf{53.3}\\
    \bottomrule
    \end{tabular}%
    }
    \vspace{-10pt}
      \caption{Summary of comparing hand-crafted models and searched models by AutoAdapt. Three variants of AutoAdapt are presented, details can be found in section \ref{sec:ablation}}
      \vspace{-15pt}
  \label{tab:summary}%
\end{table}%


==> tables/search_comp.tex <==
% Table generated by Excel2LaTeX from sheet 'table'
\begin{table}[t]
% \setlength{\abovecaptionskip}{-0.3cm} 
\setlength{\belowcaptionskip}{-0.3cm} 
%   \centering

  \resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{c|l|cc|cc}
    \toprule
    {DA} & Methods & Input Size (S) & Network depth & {mIoU(\%) $\uparrow$ } & {Search Cost$\downarrow$} \\
    \hline
   \multirow{4}[4]{*}{\rotatebox{90}{AdvEnt}}  & G-1 & 32x32 & 14    & 29.8  & 3  \\
     & G-2 & 512x256 & 5     & 30.4  &  4  \\
     & RS  & 1280*760  & 101 &   38.5 & 50 \\
     & RL & 1280*760 & 101   & \textbf{44.9}  &  200   \\
     & EA  & 1280*760 & 101   & \textbf{44.9}  & 150 \\
    %  & EA (efficient) & 1280*760 & 101   & \textbf{45.3}  & 75 \\
     \hline
     \hline
        \multirow{4}[4]{*}{\rotatebox{90}{IntraDA}}  & G-1 & 32x32 & 14    & 30.1  & 2.5 \\
     & G-2 & 512x256 & 5     & 33.9  &  3  \\
          & RS  & 1280*760  & 101 &   40.7 & 50 \\
     & RL & 1280*760 & 101   & \textbf{47.0}  &  160 \\
     & EA  & 1280*760 & 101   & 46.9  &  120 \\
    %  & EA (efficient) & 1280*760 & 101   & 46.9  &   60 \\
     \hline
     \hline
        \multirow{4}[4]{*}{\rotatebox{90}{CCM}}  & G-1 & 32x32 & 14    & 30.8  &3   \\
     & G-2 & 512x256 & 5     & 36.8  &  4  \\
          & RS  & 1280*760  & 101 &   42.1 & 50 \\
     & RL & 1280*760 & 101   & 49.9 &  200  \\
     & EA  & 1280*760 & 101   & \textbf{50.0}  & 150  \\
    %  & EA (efficient) & 1280*760 & 101   & \textbf{50.2}  & 80  \\
    \bottomrule
    \end{tabular}%
    }
    % bold font
    % & 36.8 & 38.1 49 50.1
    \vspace{-5pt}
      \caption{Comparative studies on searching algorithms. Input size is the size of source images for domain adaptation. Experiments are conducted on GTA5$\rightarrow$Cityscapes.}
      \vspace{-5pt}
  \label{tab:serach_comp}%
\end{table}%
